Chain-of-Table: Evolving Tables in the Reasoning Chain for Table Understanding

Table-based reasoning with large language models (LLMs) is a promising direction to tackle many table understanding tasks, such as table-based question answering and fact verification. Compared with generic reasoning, table-based reasoning requires the extraction of underlying semantics from both free-form questions and semi-structured tabular data. Chain-of-Thought and its similar approaches incorporate the reasoning chain in the form of textual context, but it is still an open question how to effectively leverage tabular data in the reasoning chain. We propose the Chain-of-Table framework, where tabular data is explicitly used in the reasoning chain as a proxy for intermediate thoughts. Specifically, we guide LLMs using in-context learning to iteratively generate operations and update the table to represent a tabular reasoning chain. LLMs can therefore dynamically plan the next operation based on the results of the previous ones. This continuous evolution of the table forms a chain, showing the reasoning process for a given tabular problem. The chain carries structured information of the intermediate results, enabling more accurate and reliable predictions. Chain-of-Table achieves new state-of-the-art performance on WikiTQ, FeTaQA, and TabFact benchmarks across multiple LLM choices.

==> tables/results_general_text_baseline.tex <==
\begin{table*}[htbp]
  \centering
  \small
\caption{Results of \method on WikiTableQuestions and TabFact datasets in comparison with the generic reasoning methods. The best performing method results in bold. The improvement is based on the second best method.}
\begin{tabular}{clll}
\toprule
\multirow{2}[4]{*}{\textbf{LLM}} & \multirow{2}[4]{*}{\textbf{Prompting}} & \textbf{TabFact} & \textbf{WikiTQ} \\
\cmidrule{3-4}      &       & \textbf{Accuracy} & \textbf{Accuracy} \\
\midrule
\multirow{4}[4]{*}{PaLM 2-S} & End-to-End QA & 77.92 & 60.59 \\
      & FewShot QA & 78.06 & 60.33 \\
      & Chain-of-Thought &  79.05  & 60.43  \\
\cmidrule{2-4}      & Chain-of-Table (Ours) & \textbf{86.61 \scriptsize{(+7.56)}} & \textbf{67.31 \scriptsize{(+6.72)}} \\
\bottomrule
\end{tabular}%
  \label{tab:results-general-text-baseline}%
\end{table*}%


==> tables/results_tabfact_wikitq.tex <==
\begin{table*}[htbp]
  \centering
    \small
\caption{Results of \method on WikiTableQuestions and TabFact datasets in comparison with the table-based reasoning methods. The best performing method results in bold. The improvement is based on the second best method. As reported in \citet{ye2023large}, Dater with Codex achieves 65.9 on WikiTableQuestion and 85.6 on TabFact. Because Codex is not longer avaible to the public, we cannot report the performance of \method with Codex as the LLM.}
    \begin{tabular}{clll}
    \toprule
    \multirow{2}[4]{*}{\textbf{LLM}} & \multirow{2}[4]{*}{\textbf{Prompting}} & \textbf{TabFact} & \textbf{WikiTQ} \\
\cmidrule{3-4}          &       & \textbf{Accuracy} & \textbf{Accuracy} \\
    \midrule
    \multirow{3}[2]{*}{GPT 3.5} & Binder & 79.17 & 56.74 \\
          & Dater & 78.01  & 52.81 \\
          & Chain-of-Table (Ours) & \textbf{80.20 \scriptsize{(+1.03)}} &  \textbf{59.94 \scriptsize{(+3.20)}} \\
    \midrule
    \multirow{3}[2]{*}{PaLM 2-S} & Binder & 76.98 & 54.88 \\
          & Dater & 84.63 & 61.48 \\
          & Chain-of-Table (Ours) & \textbf{86.61 \scriptsize{(+1.98)}} & \textbf{67.31 \scriptsize{(+5.83)}} \\
    \bottomrule
    \end{tabular}%
  \label{tab:results-tabfact-wikitq}%
\end{table*}%

